Self-Supervised Speech Representation Learning: A Review

Although supervised deep learning has revolutionized speech and audio processing, it has necessitated the building of specialist models for individual tasks and application scenarios. It is likewise difficult to apply this to dialects and languages for which only limited labeled data is available. Self-supervised representation learning methods promise a single universal model that would benefit a wide variety of tasks and domains. Such methods have shown success in natural language processing and computer vision domains, achieving new levels of performance while reducing the number of labels required for many downstream scenarios. Speech representation learning is experiencing similar progress in three main categories: generative, contrastive, and predictive methods. Other approaches rely on multi-modal data for pre-training, mixing text or visual data streams with speech. Although self-supervised speech representation is still a nascent research area, it is closely related to acoustic word embedding and learning with zero lexical resources, both of which have seen active research for many years. This review presents approaches for self-supervised speech representation learning and their connection to other research areas. Since many current methods focus solely on automatic speech recognition as a downstream task, we review recent efforts on benchmarking learned representations to extend the application beyond speech recognition.

==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> figures/batchsize.tex <==
ngpu km100_100k km100_100k_v1
8  38.51 38.48
16 23.98 27.82
32 17.86 22.19
% 64 0 19.97

==> figures/maskp.tex <==
maskp km100_100k km100_100k_v1
2.0 23.28 27.03
4.5 18.71 22.70
6.5 19.01 22.12
8.0 17.86 22.19
9.0 18.34 21.98

==> figures/qual_it1_km100.tex <==
layer   ref-pur    hyp-pur    H(ref)    H(hyp)      MI    MI/H(ref)    ref-segL    hyp-segL  p_xy-shape      frm-tot    frm-diff    utt-tot    utt-miss
0       0.4069     0.1260    3.3057    4.5791  1.2406       0.3753      9.6116      3.4805  (41, 100)       3776074           0       5567           0
1       0.4385     0.1410    3.3057    4.5897  1.3896       0.4204      9.6116      3.3393  (41, 100)       3776074           0       5567           0
2       0.4688     0.1543    3.3057    4.5885  1.5062       0.4556      9.6116      3.4053  (41, 100)       3776074           0       5567           0
3       0.4997     0.1837    3.3057    4.5774  1.6030       0.4849      9.6116      3.4590  (41, 100)       3776074           0       5567           0
4       0.5309     0.2135    3.3057    4.5707  1.7144       0.5186      9.6116      3.5377  (41, 100)       3776074           0       5567           0
5       0.5894     0.2686    3.3057    4.5366  1.8475       0.5589      9.6116      3.6636  (41, 100)       3776074           0       5567           0
6       0.5987     0.2735    3.3057    4.5305  1.8841       0.5700      9.6116      3.7240  (41, 100)       3776074           0       5567           0
7       0.5710     0.2739    3.3057    4.4946  1.7986       0.5441      9.6116      3.6770  (41, 100)       3776074           0       5567           0
8       0.5670     0.2559    3.3057    4.5224  1.7811       0.5388      9.6116      3.4650  (41, 100)       3776074           0       5567           0
9       0.5130     0.2025    3.3057    4.5495  1.6358       0.4948      9.6116      3.4429  (41, 100)       3776074           0       5567           0
10      0.4695     0.1760    3.3057    4.5345  1.5065       0.4557      9.6116      3.3261  (41, 100)       3776074           0       5567           0
11      0.4324     0.1867    3.3057    4.3653  1.3534       0.4094      9.6116      3.2712  (41, 99)        3776074           0       5567           0
12      0.4224     0.1445    3.3057    4.5159  1.3092       0.3960      9.6116      3.1823  (41, 100)       3776074           0       5567           0

==> figures/qual_it1_km1000.tex <==
layer     ref-pur    hyp-pur    H(ref)    H(hyp)      MI    MI/H(ref)    ref-segL    hyp-segL  p_xy-shape      frm-tot    frm-diff    utt-tot    utt-miss
0          0.4761     0.0264    3.3057    6.8496  1.5278       0.4622      9.6116      2.7506  (41, 1000)      3776074           0       5567           0
1          0.5143     0.0296    3.3057    6.8563  1.6791       0.5080      9.6116      2.6471  (41, 1000)      3776074           0       5567           0
2          0.5477     0.0329    3.3057    6.8612  1.8053       0.5461      9.6116      2.6141  (41, 999)       3776074           0       5567           0
3          0.5793     0.0363    3.3057    6.8605  1.9146       0.5792      9.6116      2.6037  (41, 1000)      3776074           0       5567           0
4          0.6397     0.0392    3.3057    6.8572  2.0912       0.6326      9.6116      2.6519  (41, 1000)      3776074           0       5567           0
5          0.6968     0.0535    3.3057    6.8147  2.2645       0.6850      9.6116      2.7959  (41, 1000)      3776074           0       5567           0
6          0.7163     0.0569    3.3057    6.7716  2.3297       0.7048      9.6116      3.0628  (41, 1000)      3776074           0       5567           0
7          0.6957     0.0668    3.3057    6.7136  2.2851       0.6913      9.6116      3.1137  (41, 1000)      3776074           0       5567           0
8          0.7073     0.0555    3.3057    6.7815  2.2929       0.6936      9.6116      2.8605  (41, 1000)      3776074           0       5567           0
9          0.6191     0.0413    3.3057    6.8385  2.0212       0.6114      9.6116      2.6860  (41, 1000)      3776074           0       5567           0
10         0.5513     0.0415    3.3057    6.7075  1.8027       0.5453      9.6116      2.7101  (41, 940)       3776074           0       5567           0
11         0.5013     0.0485    3.3057    6.4815  1.6235       0.4911      9.6116      2.6667  (41, 863)       3776074           0       5567           0
12         0.4899     0.0307    3.3057    6.7938  1.5687       0.4745      9.6116      2.5630  (41, 988)       3776074           0       5567           0
   

==> figures/qual_it1_km500.tex <==
layer     ref-pur    hyp-pur    H(ref)    H(hyp)      MI    MI/H(ref)    ref-segL    hyp-segL  p_xy-shape      frm-tot    frm-diff    utt-tot    utt-miss
0          0.4571     0.0417    3.3057    6.1758  1.4459       0.4374      9.6116      2.8988  (41, 500)       3776074           0       5567           0
1          0.4930     0.0447    3.3057    6.1796  1.5958       0.4828      9.6116      2.8069  (41, 500)       3776074           0       5567           0
2          0.5241     0.0547    3.3057    6.1782  1.7239       0.5215      9.6116      2.7644  (41, 500)       3776074           0       5567           0
3          0.5606     0.0590    3.3057    6.1771  1.8356       0.5553      9.6116      2.7649  (41, 500)       3776074           0       5567           0
4          0.6125     0.0683    3.3057    6.1691  1.9995       0.6049      9.6116      2.8427  (41, 500)       3776074           0       5567           0
5          0.6697     0.0854    3.3057    6.1351  2.1596       0.6533      9.6116      2.9836  (41, 500)       3776074           0       5567           0
6          0.6880     0.1002    3.3057    6.0900  2.2223       0.6723      9.6116      3.2658  (41, 500)       3776074           0       5567           0
7          0.6689     0.1057    3.3057    6.0388  2.1691       0.6562      9.6116      3.2397  (41, 500)       3776074           0       5567           0
8          0.6709     0.0915    3.3057    6.1161  2.1571       0.6526      9.6116      2.9698  (41, 500)       3776074           0       5567           0
9          0.5903     0.0681    3.3057    6.1551  1.9103       0.5779      9.6116      2.8390  (41, 500)       3776074           0       5567           0
10         0.5342     0.0616    3.3057    6.1249  1.7332       0.5243      9.6116      2.8329  (41, 495)       3776074           0       5567           0
11         0.4842     0.0691    3.3057    5.9003  1.5534       0.4699      9.6116      2.7788  (41, 477)       3776074           0       5567           0
12         0.4756     0.0492    3.3057    6.1362  1.5069       0.4559      9.6116      2.6840  (41, 500)       3776074           0       5567           0
   

==> figures/qual_it2_km100.tex <==
layer     ref-pur    hyp-pur    H(ref)    H(hyp)      MI    MI/H(ref)    ref-segL    hyp-segL  p_xy-shape      frm-tot    frm-diff    utt-tot    utt-miss
0          0.4109     0.1281    3.3057    4.5708  1.2828       0.3881      9.6116      3.4780  (41, 100)       3776074           0       5567           0
1          0.4484     0.1502    3.3057    4.5768  1.4472       0.4378      9.6116      3.3240  (41, 100)       3776074           0       5567           0
2          0.4774     0.1691    3.3057    4.5766  1.5442       0.4671      9.6116      3.3456  (41, 100)       3776074           0       5567           0
3          0.4999     0.1856    3.3057    4.5731  1.6099       0.4870      9.6116      3.4031  (41, 100)       3776074           0       5567           0
4          0.5225     0.2053    3.3057    4.5677  1.6779       0.5076      9.6116      3.4791  (41, 100)       3776074           0       5567           0
5          0.5629     0.2243    3.3057    4.5695  1.8109       0.5478      9.6116      3.6460  (41, 100)       3776074           0       5567           0
6          0.5878     0.2490    3.3057    4.5461  1.8739       0.5669      9.6116      3.8415  (41, 100)       3776074           0       5567           0
7          0.6026     0.2681    3.3057    4.5429  1.8968       0.5738      9.6116      3.9917  (41, 100)       3776074           0       5567           0
8          0.5721     0.2432    3.3057    4.5283  1.8224       0.5513      9.6116      4.0010  (41, 100)       3776074           0       5567           0
9          0.5523     0.2367    3.3057    4.5073  1.7917       0.5420      9.6116      3.7924  (41, 100)       3776074           0       5567           0
10         0.5807     0.2470    3.3057    4.5452  1.8601       0.5627      9.6116      3.6913  (41, 100)       3776074           0       5567           0
11         0.6002     0.2504    3.3057    4.5304  1.9202       0.5809      9.6116      3.7628  (41, 100)       3776074           0       5567           0
12         0.5808     0.2462    3.3057    4.5336  1.8810       0.5690      9.6116      4.0058  (41, 100)       3776074           0       5567           0
   

==> figures/qual_it2_km1000.tex <==
layer     ref-pur    hyp-pur    H(ref)    H(hyp)      MI    MI/H(ref)    ref-segL    hyp-segL  p_xy-shape      frm-tot    frm-diff    utt-tot    utt-miss
0          0.4865     0.0295    3.3057    6.8416  1.5824       0.4787      9.6116      2.7819  (41, 1000)      3776074           0       5567           0
1          0.5370     0.0357    3.3057    6.8490  1.7727       0.5362      9.6116      2.6362  (41, 1000)      3776074           0       5567           0
2          0.5648     0.0379    3.3057    6.8426  1.8711       0.5660      9.6116      2.5813  (41, 1000)      3776074           0       5567           0
3          0.5920     0.0382    3.3057    6.8446  1.9583       0.5924      9.6116      2.5740  (41, 1000)      3776074           0       5567           0
4          0.6235     0.0409    3.3057    6.8437  2.0436       0.6182      9.6116      2.6080  (41, 1000)      3776074           0       5567           0
5          0.6766     0.0504    3.3057    6.8267  2.2069       0.6676      9.6116      2.7201  (41, 1000)      3776074           0       5567           0
6          0.7098     0.0532    3.3057    6.8217  2.3095       0.6986      9.6116      2.8945  (41, 1000)      3776074           0       5567           0
7          0.7307     0.0563    3.3057    6.8002  2.3801       0.7200      9.6116      3.1203  (41, 1000)      3776074           0       5567           0
8          0.7200     0.0587    3.3057    6.7707  2.3606       0.7141      9.6116      3.3056  (41, 1000)      3776074           0       5567           0
9          0.7152     0.0617    3.3057    6.7490  2.3481       0.7103      9.6116      3.2599  (41, 1000)      3776074           0       5567           0
10         0.7312     0.0569    3.3057    6.7658  2.3996       0.7259      9.6116      2.9838  (41, 1000)      3776074           0       5567           0
11         0.7220     0.0582    3.3057    6.7996  2.3654       0.7156      9.6116      2.7795  (41, 1000)      3776074           0       5567           0
12         0.6933     0.0564    3.3057    6.8053  2.2724       0.6874      9.6116      2.8402  (41, 1000)      3776074           0       5567           0

==> figures/qual_it2_km500.tex <==
layer     ref-pur    hyp-pur    H(ref)    H(hyp)      MI    MI/H(ref)    ref-segL    hyp-segL  p_xy-shape      frm-tot    frm-diff    utt-tot    utt-miss
0          0.4656     0.0472    3.3057    6.1690  1.4914       0.4512      9.6116      2.9306  (41, 500)       3776074           0       5567           0
1          0.5136     0.0527    3.3057    6.1685  1.6887       0.5109      9.6116      2.7787  (41, 500)       3776074           0       5567           0
2          0.5454     0.0584    3.3057    6.1680  1.7876       0.5408      9.6116      2.7188  (41, 500)       3776074           0       5567           0
3          0.5726     0.0624    3.3057    6.1637  1.8813       0.5691      9.6116      2.7327  (41, 500)       3776074           0       5567           0
4          0.6035     0.0684    3.3057    6.1591  1.9581       0.5923      9.6116      2.7850  (41, 500)       3776074           0       5567           0
5          0.6482     0.0792    3.3057    6.1533  2.1043       0.6366      9.6116      2.9144  (41, 500)       3776074           0       5567           0
6          0.6881     0.0871    3.3057    6.1379  2.2109       0.6688      9.6116      3.1039  (41, 500)       3776074           0       5567           0
7          0.7096     0.0935    3.3057    6.1303  2.2809       0.6900      9.6116      3.3375  (41, 500)       3776074           0       5567           0
8          0.6985     0.0968    3.3057    6.1039  2.2524       0.6814      9.6116      3.5035  (41, 500)       3776074           0       5567           0
9          0.6915     0.0986    3.3057    6.0755  2.2392       0.6774      9.6116      3.4380  (41, 500)       3776074           0       5567           0
10         0.6978     0.0927    3.3057    6.1132  2.2750       0.6882      9.6116      3.2020  (41, 500)       3776074           0       5567           0
11         0.6871     0.0936    3.3057    6.1137  2.2532       0.6816      9.6116      3.1029  (41, 500)       3776074           0       5567           0
12         0.6732     0.0902    3.3057    6.1301  2.1885       0.6621      9.6116      3.2476  (41, 500)       3776074           0       5567           0


==> tables/ens.tex <==
\begin{tabular}{lc}
    \toprule
    teacher & WER \\
    \midrule\midrule
    K-means \{50,100\}       & 17.81 \\
    K-means \{50,100,500\}   & 17.56 \\
    \midrule
    Product K-means-0-100 & 19.26 \\
    Product K-means-1-100 & 17.64 \\
    Product K-means-2-100 & 18.46 \\
    Product K-means-\{0,1,2\}-100 & 16.73 \\
    \bottomrule
\end{tabular}% 

==> tables/main_hi.tex <==


\begin{table*}[t]
    \centering
    \begin{tabular}{lcccccc}
        \toprule
        Model & Unlabeled Data & LM & dev-clean & dev-other & test-clean & test-other \\
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{Superivsed}}} \\
        Conformer L~\cite{gulati2020conformer} & - & LSTM & - & - & 1.9 & 3.9 \\
        
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{Self-Training}}} \\
        IPL~\cite{xu2020iterative} & LL-60k & 4-gram + Transformer & 1.85 & 3.26 & 2.10 & 4.01 \\
        Noisy Student~\cite{park2020improved} & LV-60k & LSTM & 1.6 & 3.4 & 1.7 & 3.4 \\
        
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{Pre-Training}}} \\
        wav2vec 2.0 \textsc{Large}~\cite{baevski2020wav2vec} & LL-60k & Transformer & 1.6 & 3.0 & 1.8 & 3.3 \\
        pre-trained Conformer XXL~\cite{zhang2020pushing} & LL-60k & LSTM & 1.5 & 3.0 & 1.5 & 3.1 \\
        
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{Pre-Training + Self-Training}}} \\
        wav2vec 2.0 + self-training~\cite{xu2020self} & LL-60k & Transformer & 1.1 & 2.7 & 1.5 & 3.1\\
        pre-trained Conformer XXL + Noisy Student~\cite{zhang2020pushing} & LL-60k & LSTM & 1.3 & 2.6 & 1.4 & 2.6 \\
        
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{This work (Pre-Training)}}} \\
        HUBERT \textsc{Large}   & LL-60k & Transformer & 1.5 & 3.0 & 1.9 & 3.3 \\
        % HUBERT \textsc{X-Large} & LL-60k & Transformer & 1.6 & 2.6 & 1.8 & 3.0 \\ % old number
        HUBERT \textsc{X-Large} & LL-60k & Transformer & 1.5 & 2.5 & 1.8 & 2.9 \\
        
        \bottomrule
    \end{tabular}
    \caption{Comparison with the literature on high resource setups using all 960 hours of labeled LibriSpeech data.}
    \label{tab:main_hi}
\end{table*}


==> tables/main_lo.tex <==

\begin{table*}[t]
    \centering
    \begin{tabular}{lcccccc}
        \toprule
        Model & Unlabeled Data & LM & dev-clean & dev-other & test-clean & test-other \\
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{10-min labeled}}} \\
        % DeCoAR 2.0~\cite{ling2020decoar} & LS-960 & 4-gram & - & - & - & - \\
        DiscreteBERT~\cite{baevski2019effectiveness} & LS-960 & 4-gram & 15.7 & 24.1 & 16.3 & 25.2 \\
        wav2vec 2.0 \textsc{Base}~\cite{baevski2020wav2vec}   & LS-960 & 4-gram & 8.9 & 15.7 & 9.1 & 15.6 \\
        wav2vec 2.0 \textsc{Large}~\cite{baevski2020wav2vec}  & LL-60k & 4-gram & 6.3 & 9.8 & 6.6 & 10.3  \\
        wav2vec 2.0 \textsc{Large}~\cite{baevski2020wav2vec}  & LL-60k & Transformer & 4.6 & 7.9 & 4.8 & 8.2 \\
        \midrule
        HUBERT \textsc{Base}    & LS-960 & 4-gram & 9.1 & 15.0 & 9.7 & 15.3  \\
        HUBERT \textsc{Large}   & LL-60k & 4-gram & 6.1 & 9.4 & 6.6 & 10.1 \\
        HUBERT \textsc{Large}   & LL-60k & Transformer & 4.3 & 7.0 & 4.7 & 7.6 \\
        HUBERT \textsc{X-Large} & LL-60k & Transformer & 4.4 & 6.1 & 4.6 & 6.8 \\
        
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{1-hour labeled}}} \\
        DeCoAR 2.0~\cite{ling2020decoar} & LS-960 & 4-gram & - & - & 13.8 & 29.1 \\
        DiscreteBERT~\cite{baevski2019effectiveness} & LS-960 & 4-gram & 8.5 & 16.4 & 9.0 & 17.6 \\
        wav2vec 2.0 \textsc{Base}~\cite{baevski2020wav2vec}   & LS-960 & 4-gram & 5.0 & 10.8 & 5.5 & 11.3 \\
        wav2vec 2.0 \textsc{Large}~\cite{baevski2020wav2vec}  & LL-60k & Transformer & 2.9 & 5.4 & 2.9 & 5.8 \\
        \midrule
        HUBERT \textsc{Base}    & LS-960 & 4-gram & 5.6 & 10.9 & 6.1 & 11.3  \\
        HUBERT \textsc{Large}   & LL-60k & Transformer & 2.6 & 4.9 & 2.9 & 5.4 \\
        HUBERT \textsc{X-Large} & LL-60k & Transformer & 2.6 & 4.2 & 2.8 & 4.8 \\
        
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{10-hour labeled}}} \\
        SlimIPL~\cite{likhomanenko2020slimipl} & LS-960 & 4-gram + Transformer & 5.3 & 7.9 & 5.5 & 9.0 \\
        DeCoAR 2.0~\cite{ling2020decoar} & LS-960 & 4-gram & - & - & 5.4 & 13.3 \\
        DiscreteBERT~\cite{baevski2019effectiveness} & LS-960 & 4-gram & 5.3 & 13.2 & 5.9 & 14.1 \\
        wav2vec 2.0 \textsc{Base}~\cite{baevski2020wav2vec}   & LS-960 & 4-gram & 3.8 & 9.1 & 4.3 & 9.5 \\
        wav2vec 2.0 \textsc{Large}~\cite{baevski2020wav2vec}  & LL-60k & Transformer & 2.4 & 4.8 & 2.6 & 4.9 \\
        \midrule
        HUBERT \textsc{Base}    & LS-960 & 4-gram & 3.9 & 9.0 & 4.3 & 9.4 \\
        HUBERT \textsc{Large}   & LL-60k & Transformer & 2.2 & 4.3 & 2.4 & 4.6 \\
        HUBERT \textsc{X-Large} & LL-60k & Transformer & 2.1 & 3.6 & 2.3 & 4.0 \\
        
        \midrule\midrule
        \multicolumn{7}{c}{\textit{\textbf{100-hour labeled}}} \\
        % LPM~\cite{hsu2020semi} & LL-60K & ConvLM & 4.87 & 13.84 & 4.88 & 15.28 \\
        IPL~\cite{xu2020iterative} & LL-60k & 4-gram + Transformer & 3.19 & 6.14 & 3.72 & 7.11 \\
        SlimIPL~\cite{likhomanenko2020slimipl} & LS-860 & 4-gram + Transformer & 2.2 & 4.6 & 2.7 & 5.2 \\
        Noisy Student\cite{park2020improved} & LS-860 & LSTM & 3.9 & 8.8 & 4.2 & 8.6 \\
        DeCoAR 2.0~\cite{ling2020decoar} & LS-960 & 4-gram & - & - & 5.0 & 12.1 \\
        DiscreteBERT~\cite{baevski2019effectiveness} & LS-960 & 4-gram & 4.0 & 10.9 & 4.5 & 12.1 \\
        wav2vec 2.0 \textsc{Base}~\cite{baevski2020wav2vec}   & LS-960 & 4-gram & 2.7 & 7.9 & 3.4 & 8.0 \\
        wav2vec 2.0 \textsc{Large}~\cite{baevski2020wav2vec}  & LL-60k & Transformer & 1.9 & 4.0 & 2.0 & 4.0 \\
        
        \midrule
        HUBERT \textsc{Base}    & LS-960 & 4-gram & 2.7 & 7.8 & 3.4 & 8.1  \\
        HUBERT \textsc{Large}   & LL-60k & Transformer & 1.8 & 3.7 & 2.1 & 3.9 \\
        HUBERT \textsc{X-Large} & LL-60k & Transformer & 1.7 & 3.0 & 1.9 & 3.5 \\
        
        \bottomrule
    \end{tabular}
    \caption{Results and comparison with the literature on low resource setups (10-min, 1-hour, 10-hour, and 100-hour of labeled data).}
    \label{tab:main_lo}
\end{table*}

==> tables/model.tex <==
\begin{table*}[h!]
\caption{
The models are sorted according to publication date of the first version on arXiv which might differ from the year indicated by the citation. 
\textbc{{reg}} means that the model uses a regression loss, 
\textbc{{clf}} that it uses a classification loss,
\textbc{{con}} that it uses a contrastive loss, 
\textbc{{msk}} that it uses masking to define the target region, 
\textbc{{ltg}} that it uses a learned target, 
\textbc{{qtz}} that it uses a quantized target, and
\textbc{{emb}} that it embeds a variable length segment.
%Lee: I think contrastive always have learned target. Am I correct???
}
\label{tab:model-taxonomy}
\begin{center}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ l l | c c c | c c c | c } 
\toprule
\multicolumn{2}{c}{} & 
\multicolumn{3}{c}{\small\textsc{Loss}} & 
\multicolumn{3}{c}{\small\textsc{Target}} &
 \\
\textbc{{model}} &
\textbc{{pub. date}} &
\textbc{{reg}} & 
\textbc{{clf}} & 
\textbc{{con}} &
\textbc{{msk}} &
\textbc{{ltg}} &  
\textbc{{qtz}} & 
\textbc{{emb}} \\
\midrule
%                                                         REG      CLF      CON      MSK      LTG      QTZ      EMB  

Audio Word2vec \cite{Chung2016AudioWord2Vec}      & 2016 Mar. & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\

VQ-VAE \cite{vqvae} & 2017 Nov. & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark \\ %2 Nov 2017 

Speech2Vec \cite{chung2018speech2vec}     & 2018 Mar. & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\
Unspeech \cite{milde2018unspeech}         & 2018 Apr. & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark \\

CPC \cite{oord2018representation}         & 2018 Jul. & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark \\

PASE \cite{pascual2019learning}                   & 2019 Apr. & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark \\ % 6/4

APC \cite{chung2019unsupervised}          & 2019 Oct. & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ % 5/4

wav2vec \cite{schneider2019wav2vec}       & 2019 Apr. & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark \\ % 11/4

vq-wav2vec \cite{Baevski2020vq-wav2vec} & 2019 Oct. & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark \\ %12 Oct 2019 %Lee: vq-wav2vec is CON or CLF??? %Lee: Discrete BERT use masking, but vq-wav2vec does not It is CON, not CLF.

Discrete BERT \cite{Baevski2020vq-wav2vec,baevski2019effectiveness} & 2019 Oct. & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark \\ %12 Oct 2019 %10 Nov 2019 %In the paper of vq-wav2vec, it also includes the approach of Discrete BERT. I know this is tricky ....

Mockingjay  \cite{liu2020mockingjay}      & 2019 Oct. & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark \\ % 25/10-19


DeCoAR \cite{ling2020deep}                & 2019 Dec. & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark \\ % 3/12-19

PASE+ \cite{ravanelli2020multi}                & 2020 Jan. & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark \\ % 25/1 % I think contrastive always have learned target.

Bidir CPC \cite{kawakami2020learning} & 2020 Jan. & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark \\% 29/1

Modified CPC \cite{riviere2020unsupervised} & 2020 Feb. & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark \\ % 7/2

VQ-APC \cite{chung20e_interspeech}  & 2020 May  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark \\ %17/05

AALBERT \cite{chi2020audio}  & 2019 May & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark \\ %18 May 2020

speech-XLNet \cite{song20d_interspeech} & 2019 Oct. & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\%23 Oct 2019 %Lee: It is speech version of XLNet. I am not sure we should consider this approach has mask or not.


wav2vec 2.0 \cite{baevski2020wav2vec}     & 2020 Jun. & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark \\ % 20/6
%Lee: In my point of view, wav2vec 2.0 has learned target. The target is from the CNN encoder.

MPE \cite{liu2020masked} & 2020 May & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark \\ % 25 May 2020 %Lee: I think it has learned target. But please check.

TERA \cite{liu2021tera}                   & 2020 Jul. & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark \\ % 12/7

Speech SimCLR \cite{SpeechSimCLR} &  2020 Oct. & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark \\ %Lee: It is TERA+ SIMCLR. I considered it has learned target because contrastive always have learned target.
%27 Oct 2020

NPC \cite{liu21l_interspeech}                     & 2020 Nov. & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark \\ % 1/11

DeCoAR 2.0 \cite{ling2020decoar}          & 2020 Dec. & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark \\ % 11/12 %Lee:  DeCoAR 2.0 has VQ layer although it is not used as learning target.

wav2vec-C \cite{sadhu21_interspeech} & 2021 Mar. & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark \\ %9 Mar 2021 %Lee:  consistency loss is reconstruction

HuBERT \cite{hsu2021hubert}               & 2021 Jun. & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark \\ % 14/6

W2v-bert \cite{w2vbert} & 2021 Aug & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark \\
%7 Aug 2021

pMPC \cite{yue2021pMPC}  & 2021 Aug. & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark \\ %30 August – 3 September, 2021 (I do not find arXiv version.)

WavLM \cite{chen2021wavlm} & 2021 Oct. & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark \\ %26 Oct 2021

data2vec \cite{data2vec}     & 2022 Jan. & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark \\ % 20/1

BEST-RQ \cite{BEST-RQ} & 2022 Feb.  & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark \\ %Lee: no learned target. The target is random ...
% 3 Feb 2022

\bottomrule
\end{tabular}
\end{center}
\end{table*}


\begin{comment}
\begin{table*}[h!]
\caption{
The models are sorted according to the publication date of the first version on arXiv, which might differ from the year indicated by the citation. 
\textbc{{reg}} means that the model uses a regression loss, 
\textbc{{clf}} that it uses a classification loss,
\textbc{{con}} that it uses a contrastive loss, 
\textbc{{msk}} that it uses masking to define the target region, 
\textbc{{ltg}} that it uses a learned target, %lasseborgholt: We could consider using the inverse of this attribute. I.e., that the model uses the input as taget and belongs in the generative category.
\textbc{{qtz}} that it uses a quantized target, and
\textbc{{emb}} that it embeds a variable-length segment
}
\label{tab:model-taxonomy}
\begin{center}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ l l | c c c | c c c | c } 
\toprule
\multicolumn{2}{c}{} & 
\multicolumn{3}{c}{\small\textsc{Loss}} & 
\multicolumn{3}{c}{\small\textsc{Target}} &
 \\
\textbc{{model}} &
\textbc{{pub. date}} &
\textbc{{reg}} & 
\textbc{{clf}} & 
\textbc{{con}} &
\textbc{{msk}} &
\textbc{{ltg}} &  
\textbc{{qtz}} & 
\textbc{{emb}} \\
\midrule
%                                                         REG      CLF      CON      MSK      LTG      QTZ      EMB  
Audio Word2vec \cite{Chung2016AudioWord2Vec}      & 2016 Mar. & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\
Speech2Vec \cite{chung2018speech2vec}     & 2018 Mar. & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\
% Unspeech \cite{milde2018unspeech}         & 2018 Apr. & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark \\
CPC \cite{oord2018representation}         & 2018 Jul. & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark \\

PASE \cite{pascual2019learning}                   & 2019 Apr. & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark \\ % 6/4

APC \cite{chung2019unsupervised}          & 2019 Oct. & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ % 5/4
wav2vec \cite{schneider2019wav2vec}       & 2019 Apr. & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark \\ % 11/4
%VQ-APC \cite{chung2020vector}             & 2020 May  & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ 
Mockingjay  \cite{liu2020mockingjay}      & 2019 Oct. & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark \\ % 25/10-19
%DeCoAR \cite{ling2020deep}                & 2019 Dec. & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ % 3/12-19
%PASE+ \cite{Ravanelli2020}                & 2020 Jan. & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ % 25/1
wav2vec 2.0 \cite{baevski2020wav2vec}     & 2020 Jun. & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark \\ % 20/6
%TERA \cite{liu2021tera}                   & 2021 Jul. & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ % 12/7

NPC \cite{liu21l_interspeech}             & 2020 Nov. & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark \\ % 1/11

DeCoAR 2.0 \cite{ling2020decoar}          & 2020 Dec. & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark \\ % 11/12
HuBERT \cite{hsu2021hubert}               & 2021 Jun. & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark \\ % 14/6
data2vec \cite{data2vec}     & 2022 Jan. & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark \\ % 20/1
\bottomrule
\end{tabular}
\end{center}
\end{table*}

\end{comment}


==> tables/stability.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|ccc}
        \toprule
        \multirow{2}{*}{feature} & \multirow{2}{*}{C} 
        & \multicolumn{3}{c}{PNMI (mean $\pm$ std) with K-means Training Size = } \\
        & & 1h & 10h & 100h \\
        \midrule\midrule
        \multirow{2}{*}{MFCC}
        & 100 & 0.251 $\pm$ 0.001 & 0.253 $\pm$ 0.001 & 0.253 $\pm$ 0.001 \\
        & 500 & 0.283 $\pm$ 0.001 & 0.285 $\pm$ 0.000 & 0.287 $\pm$ 0.001 \\
        \midrule
        \multirow{2}{*}{\textsc{Base}-it1-L6}
        & 100 & 0.563 $\pm$ 0.012 & 0.561 $\pm$ 0.012 & 0.575 $\pm$ 0.008 \\
        & 500 & 0.680 $\pm$ 0.005 & 0.684 $\pm$ 0.003 & 0.686 $\pm$ 0.004 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Stability of K-means as an unsupervised unit discovery algorithm with respect to different features, numbers of clusters, and training data sizes. PNMI stands for phone-normalized mutual information.}
    \label{tab:stability}
\end{table}

==> tables/step.tex <==
\begin{tabular}{cc|cccc}
    \toprule
    \multirow{2}{*}{teacher} & \multirow{2}{*}{C} &  
    \multicolumn{4}{c}{dev-other WER (\%)} \\
    & & steps=100k & 250k & 400k & 800k \\
    \midrule
    \multirow{2}{*}{K-means}  
    & 50  & 18.68 & 13.65 & 12.40 & 11.82 \\
    & 100 & 17.86 & 12.97 & 12.32 & 11.68 \\
    \midrule
    \cite{baevski2019effectiveness} & 13.5k & \multicolumn{4}{c}{26.6} \\
    \bottomrule
\end{tabular}

==> tables/task_and_qual.tex <==
\begin{tabular}{cc|c|ccc}
    \toprule
    \multirow{2}{*}{teacher} & \multirow{2}{*}{C} & 
    \multirow{2}{*}{PNMI} &
    \multicolumn{3}{c}{dev-other WER (\%)} \\
    & & & $\alpha = 1.0$ & $\alpha = 0.5$ & $\alpha = 0.0$ \\
    \midrule\midrule
    Chenone (supervised top-line)  & 8976 & 0.809 & 10.38 & 9.16 & 9.79 \\
    \midrule
    \multirow{3}{*}{K-means on MFCC} 
    & 50  & 0.227 & 18.68 & 31.07 & 94.60 \\
    & 100 & 0.243 & 17.86 & 29.57 & 96.37 \\
    & 500 & 0.276 & 18.40 & 33.42 & 97.66 \\
    \midrule
    K-means on \textsc{Base}-it1-layer6 & 500 & 0.637 & 11.91 & 13.47 & 23.29 \\
    K-means on \textsc{Base}-it2-layer9 & 500 & 0.704 & 10.75 & 11.59 & 13.79 \\
    \bottomrule
\end{tabular}
